A Survey of Numerical Methods Utilizing Mixed Precision Arithmetic

Within the past years, hardware vendors have started designing low precision special function units in response to the demand of the Machine Learning community and their demand for high compute power in low precision formats. Also the server-line products are increasingly featuring low-precision special function units, such as the NVIDIA tensor cores in ORNL's Summit supercomputer providing more than an order of magnitude higher performance than what is available in IEEE double precision. At the same time, the gap between the compute power on the one hand and the memory bandwidth on the other hand keeps increasing, making data access and communication prohibitively expensive compared to arithmetic operations. To start the multiprecision focus effort, we survey the numerical linear algebra community and summarize all existing multiprecision knowledge, expertise, and software capabilities in this landscape analysis report. We also include current efforts and preliminary results that may not yet be considered "mature technology," but have the potential to grow into production quality within the multiprecision focus effort. As we expect the reader to be familiar with the basics of numerical linear algebra, we refrain from providing a detailed background on the algorithms themselves but focus on how mixed- and multiprecision technology can help improving the performance of these methods and present highlights of application significantly outperforming the traditional fixed precision methods.

==> spmv.tex <==
\subsection{Multiprecision Sparse Matrix Vector Product}
\label{sec:spmv}
%\team{Hartwig, Tobias}
The Sparse Matrix Vector product (SpMV) is the most fundamental operation in most sparse linear algebra algorithms. Here we want to show how well we can use \emph{lossy matrix compression} to speed up SpMV products, while still controlling the forward error.

Common IEEE number formats provide a good general-purpose representation for a large range of values, especially when the value distribution is unknown. On the other hand, for a single sparse matrix with a known, bounded value distribution, IEEE formats can provide high precision in value areas where it is not necessary, and not enough precision in areas where many values are stored. This allows us to adapt the number representation of the sparse matrix values, reducing precision in some areas where it is not necessary.

Floating point compression formats like ZFP work by using redundancies or correlations within small fixed-size blocks of data. For a generic sparse matrix stored in the CSR format, we often cannot find such correlations in the value array, as the number of non-zeros per row can vary greatly, and the order of values does not necessarily reflect locality in the underlying application problem.

We want to show the performance for a very simple lossy compression approach for a known value distribution that works by partitioning the value range into small clusters and storing only the cluster ID and residual relative to the cluster center. By representing the residuals in different storage precisions, we are able to adaptively control the per-cluster precision with which we can reconstruct the original values. A simple starting point for such a partition is a $k$-means clustering of the values of a sparse matrix.
Figure~\ref{fig:cluster-precision} shows such a clustering over a narrow value distribution for 16 and 256 clusters. By storing only the cluster index (8 bit) and residual in half precision (16 bit), we are able to reach a higher precision than by storing all values directly in single precision (32 bit) except for a few outliers around zero, where floating point formats naturally have the highest absolute precision.

This reduction in memory footprint can in turn be used to implement such an SpMV kernel efficiently on modern manycore architectures like GPUs: By storing the cluster centers in shared memory and sorting the cluster IDs by the relative precision needed to represent them accurately, we are able to adaptively control the memory footprint of an SpMV calculation against the forward-error compared to the uncompressed matrix.

\begin{figure}
\begin{tabular}{cc}
\includegraphics[scale=0.4]{graphics/cluster-precision.pdf}
&
\includegraphics[scale=0.4]{graphics/cluster-precision2.pdf}
\end{tabular}
\caption{Absolute precision for storing the values from a given distribution (dotted blue): single and double precision (dashed lines), cluster center with half precision (red) and single precision residual (green) with 16 clusters (left) and 256 clusters (right)}
\label{fig:cluster-precision}
\end{figure}
